On Stable Approximation Algorithms for Geometric Coverage Problems

Let $P$ be a set of points in the plane and let $m$ be an integer. The goal of Max Cover by Unit Disks problem is to place $m$ unit disks whose union covers the maximum number of points from~$P$. We are interested in the dynamic version of Max Cover by Unit Disks problem, where the points in $P$ appear and disappear over time, and the algorithm must maintain a set \cDalg of $m$ disks whose union covers many points. A dynamic algorithm for this problem is a $k$-stable $\alpha$-approximation algorithm when it makes at most $k$ changes to \cDalg upon each update to the set $P$ and the number of covered points at time $t$ is always at least $\alpha \cdot \opt(t)$, where $\opt(t)$ is the maximum number of points that can be covered by m disks at time $t$. We show that for any constant $\varepsilon>0$, there is a $k_{\varepsilon}$-stable $(1-\varepsilon)$-approximation algorithm for the dynamic Max Cover by Unit Disks problem, where $k_{\varepsilon}=O(1/\varepsilon^3)$. This improves the stability of $\Theta(1/\eps^4)$ that can be obtained by combining results of Chaplick, De, Ravsky, and Spoerhase (ESA 2018) and De~Berg, Sadhukhan, and Spieksma (APPROX 2023). Our result extends to other fat similarly-sized objects used in the covering, such as arbitrarily-oriented unit squares, or arbitrarily-oriented fat ellipses of fixed diameter. We complement the above result by showing that the restriction to fat objects is necessary to obtain a SAS. To this end, we study the Max Cover by Unit Segments problem, where the goal is to place $m$ unit-length segments whose union covers the maximum number of points from $P$. We show that there is a constant $\varepsilon^* > 0$ such that any $k$-stable $(1 + \varepsilon^*)$-approximation algorithm must have $k=\Omega(m)$, even when the point set never has more than four collinear points.

==> linesandpoints.tex <==
\section{No SAS for covering points by lines}
\label{sec:NOSAS for linesandpoints}

\arp{for sparse point sets, no 5 points on a line!}
Recall that in the \maxcovL problem we are given a set $P$ of points in the plane, and the goal is to find a set $\L$ of lines that covers all the points from~$P$.
%\mdb{I used $m$ instead of $k$, since $k$ is always stability. I checked
%and I think the places where we use $m$ can easily be changed to something else.} \arp{i don't immediately see anywhere that we used m, so i guess its fine? }
In this section, we prove that the dynamic version of the problem does not admit a SAS. Before we discuss the idea we first define a simple geometric representation of a graph $G$ on the plane that we refer by the \emph{sparse-line} representation of $G$.

\begin{definition}
    
\label{def:sparse-line rep}
For any graph $G$ with $n$ vertices. The embedding of $G$ in the plane such that the $n$ vertices of $G$ correspond to $n$ points in the plane (denote this set of points as $P_n$). The edges correspond to infinite lines that pass through the corresponding points in $P_n$ it is adjacent to, with the additional property that no three lines (edges) intersect at a point outside $P_n$, is called a \emph{sparse-line} representation of $G$.
\end{definition} 

It is trivial to see that for any graph $G$, a \emph{sparse-line} representation of G exists in the plane. Now observe that if the online version of the  \maxcovL problem admits a SAS, then the dual of the problem which is \hitsetL also admits a SAS. Recall that in an online construction of a graph $G$ vertices arrive one by one along with their incident edges. We now define the \emph{online-geometric} construction of a graph $G$. Fix some ordering $\sigma= \{v_1, v_2, v_3, ...\ldots v_n\}$ of the vertices of $G$. Now in the \emph{online-geometric} construction of $G$ with respect to $\sigma$, the lines of the \emph{sparse-line} representation of $G$ arrive one by one, with the only restriction that the lines corresponding to $v_j$ arrive later than the lines corresponding to $v_i$ for all $1\leq i<j\leq n$.

\subparagraph*{Idea.} We will give an overview of the idea behind the proof of the non-existence of SAS for the \emph{hitting lines by points} which in turn implies the non-existence of SAS for \emph{covering by lines}. The proof is based on the following ideas that we sketch below.

\begin{itemize}

\item Fix $0<\eps<1$. For the \emph{online-geometric} construction of a graph $G$ with minimum degree at least $3$ with respect to an ordering of the vertices $\sigma$, a $f(\eps)$-stable $1+\eps$-approximation algorithm for the \hitsetL problem, would imply the existence of a $g(\eps)$-stable, $(1+h(\eps))$-approximation algorithm for maintaining the \emph{vertex cover} when the vertices of $G$ arrive in the order $\sigma$ along with their incident edges, where $h(\eps)$ tends to $0$ as $\eps$ tends to $0$. 

    \item In the vertex arrival model, if the maximum degree of a vertex of the online graph is bounded by some constant $\Delta$, then an online algorithm of maintaining a \emph{vertex cover} for a set of instances with a good approximation ratio and bounded stability will imply the existence of an online algorithm for maintaining \emph{independent set} with good approximation ratio and good stability for the same set of instances.

\item Based on the idea of using expander graphs in~\cite{DBLP:conf/approx/BergSS23} to show non-existence of SAS for the independent set problem, we give an alternate construction ($G^*$) for the same using almost identical ideas. The only difference is that, in our construction, the minimum degree of every vertex is at least $3$ (which is necessary for our proof to work), which was not the case for the construction used in~\cite{DBLP:conf/approx/BergSS23}.

\item Now, we do an \emph{online-geometric} construction of $G^*$ to arrive at a contradiction using the ideas above.


\end{itemize}. 



\subparagraph*{Vertex cover to Independent Set.}
Recall that a vertex cover of a graph is a set of vertices that includes at least one endpoint of every edge of the graph. An independent set is a set of vertices in a graph, no two of which are adjacent. It is easy to see that a set of vertices is a vertex cover if and only if its complement is an independent set. We first observe a simple lemma below that connects the size of the complement of an approximate vertex cover to the size of the optimal independent set.

\begin{lemma}\label{lem:VCtoIS}
    Suppose $G$ is a graph with maximum degree $\Delta$ and let $\opt_{vc}(G), \opt_{I}(G)$ denote the optimal vertex cover and independent set of $G$ respectively. Let $S$ be a vertex cover of $G$ such that $|S| \leq (1+\eps)\cdot|\opt_{vc}(G)|$ for some constant $\eps>0$. Then $S^c$, the complement of $S$ is an independent set of $G$ satisfying $(1-(\Delta-1)\cdot \eps)|\opt_{I}(G)|\leq |S^c|$.
    
\end{lemma}

\begin{proof}
Since maximum degree is bounded by $\Delta$, we know that $\opt_{I}(G)  \geq  \frac{n}{\Delta}$, thus  $\opt_{vc}(G)  \leq  n-n/ \Delta \leq (\Delta-1)\opt_{I}(G) $. Now as $|S| \leq  (1+\eps)\cdot|\opt_{vc}(G)$, we have
\[
\begin{array}{lll}
 n-|S|=|S^c| & \geq & n- [(1+\eps)\cdot|\opt_{vc}(G)|]  \\
 & \geq & |\opt_{I}(G)| -[\eps \cdot|\opt_{vc}(G)|]  \\
      & \geq & (1-(\Delta-1)\eps) \cdot \opt_{I}(G)) \\
     .
\end{array}
\]

\end{proof}

In the context of dynamic algorithms, in the vertex arrival model where $G(t)$ denotes the dynamic graph at time $t$, we already know that even if the maximum degree of a vertex is bounded by $3$ at all times, there does not exist a SAS for the independent set problem~\cite{DBLP:conf/approx/BergSS23}.
We note some easy corollaries of this fact combined with the above lemma below. 
 

\begin{corollary} \label{cor:VCtoIC}
    If there exists an $f(\eps)$-stable, $(1+\eps)$-approximation algorithm $\alg$, that maintains a vertex cover till $t=N$. Then the algorithm that outputs the complement of the output of $\alg$ is a $f(\eps)$-stable, $(1+(\Delta-1)\eps)$-approximation algorithm for the independent set till $t=N$.
\end{corollary}



\begin{corollary} A SAS for the vertex cover problem when the maximum degree of G(t) is bounded by $\Delta$ implies a SAS for the Independent set problem when the maximum degree of G(t) is bounded by $\Delta$. Thus for $\Delta \geq 3$, the vertex cover problem does not admit a SAS.
\end{corollary}


\subparagraph*{No SAS for Independent set using expander graphs, an alternative construction.}
Berg~\etal~\cite{DBLP:conf/approx/BergSS23} showed using an expander construction that there is no SAS even when the dynamic graphs are restricted to being bipartite and having a maximum degree of $3$. In this paper, we use the same idea but a slightly modified construction that will be used to prove no SAS for our \maxcovL problem \arp{even when...}.



We now give the modified expander construction that proves a no SAS for dynamic graphs that are restricted to being bipartite and having a maximum degree of $4$ and minimum degree 3.


The Lemma on the existence of a 3-regular expander graph is well known. For a nice survey of expander graphs, we refer the reader to~\cite{Linial2006ExpanderGA}.

\begin{lemma} \label{thm:property of bipartite expander}
For any $n\in \mathbb{N}$ large enough, there exists a 3-regular bipartite graph $H$=($L \cup R$) with $|L=|R|=n$, and a constant $0 < \alpha <1$ such that, for all sets $S\subseteq L$ of at most $\alpha n$ vertices, $N(S)\subseteq R$ has size at least $1.99\cdot|S|$.
\end{lemma}

Let $\eps:=\min \left(\frac{\alpha}{384-\alpha}, \frac{2-\alpha}{16+\alpha}\right)$. We suppose there exists an $\alg$ that maintains an approximation ratio of $1+\eps$ and has a stability parameter bounded by $k_{\eps}$. Choose a natural number $n$ such that $k_{\eps} \leq \frac{1}{384}\lfloor{\alpha n}\rfloor$.
Now we construct a graph $G$ in an online manner. Let $G_t$ be the online graph formed after arrival of the $t^{th}$ vertex. Let $I_{\alg}(t)$ be the set of vertices in the output independent set of $\alg$ after arrival of the $t^{th}$ vertex. Also let $I_{\opt}(t)$ be the set of vertices in a maximum independent set of $G_t$. We will show the impossibility of existence of SAS using the construction of a series of insertions below which is inspired from the expander graph H.\newline

\emph{Construction of the graph $G(t)$ in an online manner:} \label{counterexampleconstruction}

\begin{itemize}
    \item First $|R|=n$ number of isolated vertices arrive one by one from $t=1$ to $n$. 
    \item Next the vertices $l_i \in L$, $i=\{1, 2, \ldots, n\}$ along with their corresponding three edges arrive one by one.
    \item Then $\lfloor{\frac{n}{4}}\rfloor$ number of new degree $3$ vertices arrive one by one and each of them is connected to distinct $3$ vertices in $R$. We denote this set of vertices by $S$.

    \item Let $G^*$ denote the final graph at $t=2n+\lfloor{\frac{n}{4}}\rfloor$, with vertex set $L \cup R\cup S$.
\end{itemize}


Observe that after $2n$ steps we have a realization of the graph $H$ which is formed in an online manner. Then a few more degree $3$ vertices arrive that have edges adjacent to $R$. Note that it is possible to construct in a way such that no two vertices in $S$ share a common neighbor as the cardinality of $S$ is strictly less than $n/3$. 



\begin{observation}
If $t \leq 2n$, then the degree of every vertex of $G(t)$ is less than or equal to $3$. And $2n<t \leq \lfloor{\frac{n}{4}}\rfloor$, the degree of every vertex of the $G(t) \cap L \cup S$ is less than or equal to $3$ and the degree of every vertex of the $G(t) \cap R$ is less than or equal to $4$. 
    
\end{observation}

\begin{lemma} \label{thm:property of construction}
If the approximation ratio is bounded by $1+\eps$ then the number of vertices in $I_{\alg}(t) \cap (L \cup S)$ is strictly less than $\frac{\alpha n}{16}$ for all $t=n+1, n+2, n+3, \ldots , 2n+ \lfloor{\frac{n}{4}}\rfloor$.
\end{lemma}
\begin{proof}
For the sake of contradiction assume $t_f$ to be the first time in which $|I_{\alg}(t_f) \cap (L \cup S)| \geq \frac{\alpha n}{16}$. Clearly as the stability parameter of $\alg$ is equal to $k_\eps$, we have that at time $t_f$, $|I_{\alg}(t_f) \cap (L \cup S)| \leq \frac{\alpha n}{16} + k_\eps$. Let $I_{\alg}(t_f) \cap L=V_1$ and $I_{\alg}(t_f) \cap S=V_2$. We do the following case distinction

\emph{Case 1:} If $|V_1| \geq \frac{7}{12} \cdot \frac{\alpha n}{16}$, then by  theorem \ref{thm:property of bipartite expander} we have $N(V_1)>\frac{13}{12} \cdot \frac{\alpha n}{16}$. Hence cardinality of $|I_{\alg}(t_f) \cap R| \leq n-\frac{13}{12} \cdot \frac{\alpha n}{16}$. Hence $|I_{\alg}(t_f)|=|I_{\alg}(t_f) \cap R| + |I_{\alg}(t_f) \cap (L \cup S)| \leq  \frac{\alpha n}{16} + k_\eps + n-\frac{13}{12} \cdot \frac{\alpha n}{16} =k_\eps + n-\frac{1}{12} \cdot \frac{\alpha n}{16} <n- \frac{\alpha n}{384}$. Hence the approximation ratio maintained by $\alg$ at time $t_f$ is strictly greater than $\frac{n}{n- \frac{\alpha n}{384}}=1+\frac{\alpha}{384-\alpha} \geq 1+\eps$ which is a contradiction.

\emph{Case 2:} If $|V_1| < \frac{7}{12} \cdot \frac{\alpha n}{16}$, then we have $|V_2| \geq \frac{5}{12} \cdot \frac{\alpha n}{16}$. So by construction we have $N(V_2)>\frac{15}{12} \cdot \frac{\alpha n}{16}$. Hence cardinality of $|I_{\alg}(t_f) \cap R| \leq n-\frac{15}{12} \cdot \frac{\alpha n}{16}$. Hence $|I_{\alg}(t_f)|=|I_{\alg}(t_f) \cap R| + |I_{\alg}(t_f) \cap (L \cup S)|$ and now $|I_{\alg}(t_f) \cap R|$ is even lesser than in \emph{Case 1}, so we have that the approximation ratio maintained by $\alg$ at time $t_f$ is strictly greater than $1+\eps$ which is again a contradiction.

Hence we have our theorem.
\end{proof}

\begin{theorem} \label{thm:NOSASIS}
$\alg$ cannot maintain an approximation ratio of $1+\eps$. Hence we have no SAS for the online arrival model in which all vertices of the online graph has degree less than or equal to $4$ at all times.
\end{theorem}
\begin{proof}
Let $t=2n+ \lfloor{\frac{n}{4}}\rfloor$, then by lemma \ref{thm:property of construction} we have $|I_{\alg}(t) \cap (L \cup S)| \leq \frac{\alpha n}{16}$, also $|I_{\alg}(t) \cap R| \leq n$. So we have $|I_{\alg_{t}}|=|I_{\alg_{t}} \cap R| + |I_{\alg_{t}} \cap (L \cup S)| \leq n+ \frac{\alpha n}{16}$. Hence the approximation ratio $\frac{I_{\opt}(t)}{I_{\alg}(t)} > \frac{n+n/8}{n+ \alpha n/16}=\frac{18}{16+\alpha}=1+\frac{2-\alpha}{16+\alpha} \geq 1+\eps$ which is a contradiction.
\end{proof}


\subparagraph*{From geometric hitting set to non-geometric vertex cover to Independent Set.}
We now do the \emph{online-geometric} construction of $G^*$ (the graph~[\ref{counterexampleconstruction}] used for proving the non-existence of SAS for the independent set) with respect to some fixed ordering of the vertices $\sigma$ in an online manner. We will show that if there exists an $f(\eps)$-stable, $1+\eps$-approximation algorithm for the \emph{hitting lines by points} for this particular set of instances, then we can maintain a $1+\eps$-approximation algorithm for the vertex cover with a stability of $6f(\eps)$ \arp{check} for the set of instances where vertices of the graph $G^*$ arrive one by one along with their incident edges with respect to an ordering $\sigma'$ derived from $\sigma$ (the ordering used in the \emph{online-geometric} construction of $G^*$). Thus we will arrive at a contradiction by Corollary~\ref{cor:VCtoIC} and Theorem~\ref{thm:NOSASIS}.

With slight abuse of notation, we denote the \emph{sparse-line} representation of $G^*$, the final graph in the construction used for proving non-esistence of SAS for independent set~[\ref{counterexampleconstruction}] as $G^*$. Let $L= \{l_i, 1 \leq i \leq n\}$ $R= \{r_i, 1 \leq i \leq n\}$ denote the left and right points (vertices) of $G^*$. Let $S= \{s_i, 1 \leq i \leq \lfloor{\frac{n}{4}}\rfloor \}$. 

Without loss of generality, we slightly modify the \emph{online-geometric} construction of $G^*$ with respect to the ordering $\sigma=\{l_1,l_2,l_3, \ldots l_n, s_1,s_2, \ldots, s_j, r_1, r_2, r_3, \ldots r_n\}$ below (here $j=\lfloor{\frac{n}{4}}\rfloor $).
\begin{itemize}
    \item Let lines arrive three at a time such that at $t=i$, all the lines adjacent to $l_i$ arrives for all $i=1,2 \ldots,n$. 

    \item Again lines arrive three at a time such that at $t=n+k$, all the lines adjacent to $s_k$ arrives for all $k=1,2 \ldots, \lfloor{\frac{n}{4}}\rfloor$. (Note that after this there are no lines left in the \emph{sparse-line} representation of $G^*$.)

\end{itemize}

It is easy to observe that a $f(\eps)$-stable, $1+\eps$-approximation algorithm for the \emph{hitting lines by points} for this particular set of instances when instead of three lines coming together, one line comes at a time (maintaining the order of arrival \arp{how to write properly?}), translates to a $3f(\eps)$-stable, $1+\eps$-approximation algorithm for this new model of arrival. Note that the vertices of $G^*$ will be also denoted as points in the plane whenever applicable, for example, by points in $L$, we refer to the points on the plane that correspond to the vertices in $L$ in the \emph{sparse-line} representation of $G^*$. 

%Also, note that in the construction of $G^*$, we can assume n as large as we want, in particular assume $n > f(\eps)/\eps$.

Let the intersection of the lines of $G^*(t)$ outside the points $L \cup R \cup S$ be denoted by the set $Bad(t)$. Also denote any point at time $t$ belonging to  $L \cup R \cup S$ to be $Good(t)$. Let $\alg$ be a $1+\eps$-approximation algorithm with stability at most $f(\eps)$ for the \emph{hitting lines by points} for the instances when we have an \emph{online-geometric} construction of $G^*(t)$. Let $\opt_{\mathrm{hs}}(t)$ and $\alg_{\mathrm{hs}}(t)$ denote the optimal hitting set and the hitting set maintained by the algorithm respectively at time $t$.

\begin{observation}~\label{obs:optestimate}
    $\opt_{\mathrm{hs}}(t)=t$ for all  $t=1,2 \ldots,n$. And $\opt_{\mathrm{hs}}(t) = n$ for $t \geq n$. 
\end{observation}

\begin{proof}
   If $t \leq n$, then the points in $L \cap V(G^*(t))$ form a hitting set, and if $t>n$, the points in $R$ form a hitting set. Hence by the \emph{online-geometric} construction of $G^*$, the proof follows.
\end{proof}

\begin{theorem}~\label{thm:good is good enough}
    
$|Bad(t) \cap \alg_{\mathrm{hs}}(t)| \leq 9\eps \cdot \opt_{\mathrm{hs}}(t)$ for all $t=1,2, \ldots 2n+\lfloor{\frac{n}{4}}\rfloor$.

\end{theorem}
\begin{proof}
    

Suppose contradiction and assume that there exists $t^*$ such that $|Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*)|=9\eps \opt_{\mathrm{hs}}(t^*)+x$, with $x>0$. So the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps \opt_{\mathrm{hs}}(t^*)+2x$.

We also know that, $|\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$. This implies
$$|Good(t^*) \cap \alg_{\mathrm{hs}}(t^*)|+|Bad(t^*) \cap\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$$
$$\implies |Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)| \leq (1-8\eps)|\opt_{\mathrm{hs}}(t^*)|-x$$

We divide the proof into two cases.

\emph{Case 1: $t^*\leq n$:} Clearly all vertices of $G(t^*)$ have degree less than or equal to 3. Thus the number of lines hit by points in $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ is less than or equal to $3(1-8\eps)t^*-3x$. Hence the total number of lines hit by $\alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)t^*-3x+ 18\eps t^*+2x<3t^*$. This gives a contradiction as the number of edges of $G(t^*)$ is exactly equal to $3t^*$.

\emph{Case 2: $t^*> n$:} By Observation~\ref{obs:optestimate}, we have that the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps n+2x$. Also, $|Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)n-x$. Consider the set $S$ of $3n$ lines that arrive till $t=n$. Observe that any point of $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ hits at most $3$ lines of $S$. Thus the number of lines in $S$ that are hit by some point in $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)n-3x$. Hence the total number of lines of $S$ hit by $\alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)n-3x+ 18\eps n+2x<3n$. This gives a contradiction. 

This finishes the proof.


\end{proof}


Now consider the vertex arrival model, in which vertices of the graph $G^*$ arrive in the order $\sigma'=\{l_1,l_2,l_3, \ldots l_n, s_1,s_2, \ldots, s_j, r_1, r_2, r_3, \ldots r_n\}$. We describe this below. \newline


\emph{Construction of the graph $G^*$ in the vertex arrival model with respect to $\sigma'$:} \label{counterexampleconstruction1}

\begin{itemize}
    \item First $|R|=n$ number of isolated vertices arrive one by one from $t=1$ to $n$. 
    \item Next the vertices $l_i \in L$, $i=\{1, 2, \ldots, n\}$ along with their corresponding three edges arrive one by one.
    \item Then $\lfloor{\frac{n}{4}}\rfloor$ number of new degree $3$ vertices arrive one by one and each of them is connected to distinct $3$ vertices in $R$. We denote this set of vertices by $S$.
\end{itemize}

Let $G(t)$ be the graph at time $t$ with vertex set $V(t)$ defined above.


\begin{observation}\label{obs:pointtovertex}
    The set of vertices of $G^*$ that represents the points in $Good(t)$ (in the \emph{online-geometric} construction of $G^*$) is a subset of $V(t+n)$.
\end{observation}

With slight abuse of notation, for $t>n$, in the vertex arrival model, we call the set of vertices of $G^*$ that represents the points in $Good(t-n)$ (in the \emph{online-geometric} construction of $G^*$), as $Good(t)$. Also, note that the lines at time $t$ in the \emph{online-geometric} construction of $G^*$ correspond to the edges at time $t+n$ in the vertex arrival construction of $G^*$. 

Observe that the optimal vertex cover till $t=n$ is an empty set. At $t>n$, define the set $Good^*(t)$ to be the union of the vertices that are end-points of the edges that are hit by points in $Bad(t-n) \cap \alg_{hc}(t-n)$. 

\begin{observation}\label{obs:cardinalityofGood*}
$|Good^*(t)| \leq 2|Bad(t') \cap \alg_{hc}(t')|.$
   \end{observation}

\begin{lemma}\label{lemma:VCapproximation}
$Good^*(t) \cup Good(t)$ forms a vertex-cover of $G^*(t)$ for $t>n$.
   \end{lemma}
\begin{proof}
    \arp{trivial}
\end{proof}

\begin{lemma}\label{lemma:VCapproximation}
The algorithm for vertex cover that outputs an empty set for $t \leq n$ and outputs the set of vertices $Good^*(t) \cup Good(t)$ for $t>n$ is a $2f(\eps)$-stable, $1+10\eps$-approximation algorithm for the vertex-cover for this set of instances.
   \end{lemma}
\begin{proof}
    \arp{not hard}
\end{proof}




\arp{after this just relate this to no sas for ind set to get our final theorem....5 lines max.. }













%\begin{theorem}~\label{thm:good is good enough}
    
%$|Bad(t) \cap \alg_{\mathrm{hs}}(t)| \leq 9\eps \opt_{\mathrm{hs}}(t)$ for all $t>f(\eps)/\eps$.

%\end{theorem}
%\begin{proof}
    

%Observe that at $t=1$, $|Bad(t)|=0$. Suppose contradiction and let $t^*>f(\eps)/\eps$ be the first time such that $|Bad(t)\cap \alg_{\mathrm{hs}}(t)|>9\eps \opt_{\mathrm{hs}}(t)$. Hence clearly, $|Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*)|\leq 9\eps \opt_{\mathrm{hs}}(t)+3f(\eps)$. So the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps \opt_{\mathrm{hs}}(t^*)+6f(\eps)$.

%We also know that, $|\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$. This implies
%$$|Good(t^*) \cap \alg_{\mathrm{hs}}(t^*)|+|Bad(t^*) \cap\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$$
%$$\implies |Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)|\opt_{\mathrm{hs}}(t^*)|$$

%We divide the proof into two cases.

%\emph{Case 1: $t^*<n$:} Here we have that the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps t^*+6f(\eps)$. Also, $|Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)t^*$. Since $t^*<n$, all vertices of $G(t^*)$ have degree less than or equal to 3. Thus the number of lines hit by points in $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ is strictly less than $3(1-8\eps)t^*$. Hence the total number of lines hit by $\alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)t^*+ 18\eps t^*+6f(\eps)=3t^*-6(\eps t^*-f(\eps))$. 

%Additionally, we know that the number of edges of $G(t^*)$ is exactly equal to $3t^*$. Thus we have $6(\eps t^*-f(\eps)) \leq 0$. This implies $t^* \leq f(\eps)/\eps$. Thus we have a contradiction.

%\emph{Case 2: $t^*\geq n$:} By Observation~\ref{obs:optestimate}, we have that the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps n+6f(\eps)$. Also, $|Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)n$. Consider the set $S$ of $3n$ lines that arrive till $t=n$. Observe that any point of $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ hits at most $3$ lines of $S$. Thus the number of lines in S that are hit by some point in $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)n$. Hence the total number of lines of $S$ hit by $\alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)n+ 18\eps n+6f(\eps)=3n-6(\eps n-f(\eps))$. 

%Thus we have $6(\eps n-f(\eps)) \leq 0$. This implies $n \leq f(\eps)/\eps$. Thus we have a contradiction.


%\end{proof}


%\begin{theorem}
    
%$|Bad(t) \cap \alg_{\mathrm{hs}}(t)| \leq \max \{9\eps \opt_{\mathrm{hs}}(t), {3f(\eps)/\eps\choose 2}\}$ for all $t=1,2, \ldots 2n+\lfloor{\frac{n}{4}}\rfloor$.

%\end{theorem}
%\begin{proof}
    

%Observe that at $t=1$, $|Bad(t)|=0$. Suppose contradiction and let $t^*>1$ be the first time such that $|Bad(t)\cap \alg_{\mathrm{hs}}(t)|>\max \{9\eps \opt_{\mathrm{hs}}(t), {3f(\eps)/\eps\choose 2}\}$. Hence clearly, $|Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*)|\leq \max \{9\eps \opt_{\mathrm{hs}}(t), {3f(\eps)/\eps\choose 2}\}+3f(\eps)$. So the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps \opt_{\mathrm{hs}}(t^*)+6f(\eps)$.

%We also know that, $|\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$. This implies
%$$|Good(t^*) \cap \alg_{\mathrm{hs}}(t^*)|+|Bad(t^*) \cap\alg_{\mathrm{hs}}(t^*)| \leq (1+\eps)|\opt_{\mathrm{hs}}(t^*)|$$
%$$\implies |Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)|\opt_{\mathrm{hs}}(t^*)|$$

%We divide the proof into two cases.

%\emph{Case 1: $t^*<n$:} Here we have that the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps t^*+6f(\eps)$. Also, $|Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)|< (1-8\eps)t^*$. Since $t^*<n$, all vertices of $G(t^*)$ have degree less than or equal to 3. Thus the number of lines hit by points in $Good(t^*)\cap \alg_{\mathrm{hs}}(t^*)$ is strictly less than $3(1-8\eps)t^*$. Hence the total number of lines hit by $\alg_{\mathrm{hs}}(t^*)$ is less than $3(1-8\eps)t^*+ 18\eps t^*+6f(\eps)=3t^*-6(\eps t^*-f(\eps))$. 

%Additionally, we know that the number of edges of $G(t^*)$ is exactly equal to $3t^*$. Thus we have $6(\eps t^*-f(\eps)) \leq 0$. This implies $t^* \leq f(\eps)/\eps$. Thus the number of points in $Bad(t^*)$ is bounded by ${3t^* \choose 2}={3f(\eps)/\eps \choose 2}$ (As bad points are formed by the intersection of some two lines). Thus we have a contradiction.

%\emph{Case 2: $t^*\geq n$:} By observationHere we have that the number of lines hit by points in $Bad(t^*)\cap \alg_{\mathrm{hs}}(t^*) \leq 18\eps t^*+6f(\eps)$.



%\arp{i think i have a proof I am too tired to write, its a bit tricky i think}
%\arp{i will write when i wake up, i hope i am not wrong}

%\end{proof}



==> original_version.tex <==
\mdb{The original version.}
Algorithm \textsc{Partition-Creation} described below creates a partition $\mathcal{P}(i)=\{P^i_1, P^i_2, \ldots P^i_{m_i}\}$ of $\mathcal{B}$.  
\begin{algorithm}[H] 
\caption{\textsc{Partition-Creation}($\mathcal{B}, i, c$)}
\begin{algorithmic}[1]
\State $j=1, d=1$
\While{$j \leq |\mathcal{B}|=m$} 
       \State \parbox[t]{125mm}{Set $P^i_1=\bigcup_{k=1}^{i}Bl(k)$, Set j=j+i and $d=d+1$}
       \State \parbox[t]{125mm}{If $m-j+1 \geq c$, Set $P^i_d=\bigcup_{k=j}^{j+c-1} Bl(k)$, Set $j=j+c$ and $d=d+1$. }
       \State \parbox[t]{125mm}{If $m-j+1 < c$, Set $P^i_d=\bigcup_{k=j}^{m} Bl(k)$. Set $j=m+1$}       
 \EndWhile
\end{algorithmic}
\end{algorithm}
Let $c=\lceil \frac{4(2z+2)}{\varepsilon}\rceil+1$ be a constant where $z=\lceil 6c^*\rceil+4$. Let us consider $c$ different partitions of $\mathcal{B}$ namely $\mathcal{P}(i)$, $1\leq i \leq c$.
Now to form the groups we will attach a few more blocks to each part of every partition.

Let $I(P^i_j)=\max\{p: Bl(p) \in P^i_j\}$. Observe that from algorithm \textsc{partition-creation}, we have $I(P^i_j)=i+(j-1)c$ if $j\leq m_i-1$ and $I(P^i_{m_i})=m$.  

We define \[R^i_j=\bigcup_{p=I(P^i_j)+1}^{I(P^i_j)+z-1} Bl(p)\] for all $1\leq i \leq c$ and $1\leq j\leq m_i-2$. Note that it is well defined as $j \leq m_i-2$ implies $I(P^i_j)+z-1 \leq m$.

\arp{Note that I had to define the last two remainders differently as there may not be enough blocks left at the end of a partition}


We also define \[R^i_{m_i}=R^i_{m_i-1}=\bigcup_{p=z(i-1)+1}^{zi} Bl(p)\]. It is also well-defined as $z \times i \leq m$. We call $R^i_j$ to be the remainder of $P^i_j$. Let us define $Q^i_j=P^i_j \cup R^i_j$, for all $1\leq i \leq c$ and $1\leq j\leq m_i$. We call  $Q^i_j$ as a group. Define \[D_{\alg}(t-1, Q^i_j)=\bigcup_{X\in Q^i_j} D_{\alg}(t-1, C) \], where X denotes the cells within the blocks present in $Q^i_j$. Similarly, we define \[\cDoptin(t, P^i_j)=\bigcup_{X\in P^i_j} \cDoptin(t, C) \].

Remember that $k$ is the number of disks used by the algorithm to cover points \arp{have to fix a symbol other than k for this}. Also assume that $k>\frac{c^*+2}{\varepsilon^2}(z+2)c$, otherwise choosing $f(\varepsilon)=2k=O(\frac{1}{\varepsilon^3})$ will be enough to maintain an optimal solution at all times. So, by property 1 of a block, we have, $m>\frac{k}{\frac{c^*+2}{\varepsilon^2}}>(z+2)c$. 

\begin{observation} \label{disjoint remainder}
  $R^i_j \cap P^i_j=\emptyset$ for all $1\leq i \leq c$ and $1\leq j\leq m_{i}$
\end{observation}

\begin{proof}
 For $j\leq m_i-2$ it directly follows from the definition. Now assume $j>m_i-2$. By construction in \textsc{partition-creation} it follows that if $Bl(p) \in P^i_j$ then $p \geq m-2c$. Now if $Bl(p) \in R^i_j$ then $p \leq zc$. Now since $m-2c>zc$, we have our observation.
\end{proof}

\begin{lemma} \label{possiblereplacement}
   $|D_{\alg}(t-1, Q^i_j)| \geq |\cDoptin(t, P^i_j)|$ for all $1\leq i \leq c$ and $1\leq j\leq m_i$.
\end{lemma}

\begin{proof}
   Observe that $P^i_j$ is a union of consecutive blocks of $\mathcal{B}$. Hence by triangle inequality and Lemma~\ref{property of block rearrangement}, we have  $|\cDoptin(t, P^i_j)|-|D_{\alg}(t-1, P^i_j)| \leq \frac{6c^*+4}{\varepsilon^2}$. Now  $R^i_j$ consists of $z=\lceil (6c^*+4)c^*\rceil$ blocks. Hence from property 1 of a block and observation~\ref{disjoint remainder}, we have, $$|\cDoptin(t, P^i_j)|-|D_{\alg}(t-1, Q^i_j)|=|\cDoptin(t, P^i_j)|-(|D_{\alg}(t-1, P^i_j)|+|D_{\alg}(t-1, R^i_j)|)\leq 0$$. This finishes our proof.
\end{proof}

We first state the well-known Quotient-Remainder theorem in elementary number theory.

\begin{theorem} \label{quotient-reaminder}
    Given any integer $n$ and positive integer $d$, there exist unique integers $q$ and $r$ such that $n =dq+r$ and $0\leq r <d$.
\end{theorem}

\begin{lemma} \label{size of remainder(1)}
 Fix a natural number $1 \leq p \leq m$. Then the number of tuples $(i,j)$ with $1\leq i \leq c$ and $1\leq j\leq m_{i}-2$, such that $Bl(p)\in R^i_j$ is bounded by $2z$.
\end{lemma}
\begin{proof}
  Since  $j\leq m_{i}-2$ and $z<c$, it is clear from the definition of $R^i_j$ that $Bl(p)\in R^i_j$ iff $p=i+(j-1)c+r$ where $r \leq z$ is some natural number and $1\leq j\leq m_{i}-2$. Now fix a value of $r \leq c$ and suppose $(p-r)=(j-1)c+i$. Now if $i=c$, $(p-r)=(j-1)c+i$ implies $j=(p-r)/c$. So if $i=c$ , there is at most one tuple $(i,j)$ satisfying the equation $(p-r)=(j-1)c+i$, depending on whether $(p-r)/c$ is an integer or not. 
Now suppose $i<c$. Observe that $(p-r)$ and $c$ are fixed positive natural numbers. Since $0\leq i<c$, by Theorem~\ref{quotient-reaminder}, we have a unique tuple $(i,j)$ for which the equation $(p-r)=(j-1)c+i$ is satisfied. Hence for $i<c$ there is at most one tuple $(i,j)$ for which the equation $(p-r)=(j-1)c+i$ is satisfied. So for a fixed value of $r$, there are at most $2$ tuples $(i,j)$ for which the equation $(p-r)=(j-1)c+i$ is satisfied. Since there are $z$ many possible values of $r$ there are at most $2z$ tuples $(i,j)$ with $1\leq i \leq c$ and $1\leq j\leq m_{i}-2$, such that $Bl(p)\in R^i_j$.


\end{proof}

\begin{lemma} \label{size of remainder(2)}
 Fix a natural number $1 \leq p \leq m$. Then the number of tuples $(i,j)$ with $1\leq i \leq c$ and $j=m_{i}-1 \; \text{or} \; m_{i}$, such that $Bl(p)\in R^i_j$ is at most $2$.
\end{lemma}
\begin{proof}
    Let $j=m_{i}-1$. So we have, $Bl(p)\in R^i_j$ iff $z(i-1)+1 \leq p \leq zi$. Now as $z, p$ are fixed natural numbers, there is at most one value of $i$ such that $z(i-1)+1 \leq p \leq zi$. The case is exactly the same when  $j=m_{i}$ hence the lemma follows.
\end{proof}



Consistent with our previous definitions we let 
$P^*(\cDoptin(t, P^{i}_{j}))=P(\cDoptin(t, P^{i}_{j})) \setminus P(\partial\cDalg(t-1))$ denote the set of points covered by the interior unit disks of the optimal solution that are present in $P^{i}_{j}$ minus any point covered by a boundary disk of the algorithm at time $t-1$.


\begin{lemma} \label{Swapping increase number of point}
   There exists $i,j$ with $1\leq i^* \leq c$ and $1\leq j^*\leq m_{i^*}$ such that $|P^*(\cDoptin(t, P^{i^*}_{j^*}))|> |P(D_{\alg}(t-1, Q^{i^*}_{j^*}))|$.
\end{lemma}

\begin{proof}
Observe that by Lemma~\ref{lem:remaining opt} and construction, we have,  $$\sum_{(i,j)}|P^*(\cDoptin(t, P^{i}_{j}))|=c|P^*(\cDoptin(t))| \geq (c+\frac{c\varepsilon}{4})|\alg(t-1)|$$, where the sum runs over all pairs $(i,j)$ with $1\leq i \leq c$ and $1\leq j \leq m_{i^*}$. 

Now by Observation~\ref{disjoint remainder}, we know $$|P(D_{\alg}(t-1, Q^{i}_{j}))|=|P(D_{\alg}(t-1, P^{i}_{j}))|+|P(D_{\alg}(t-1, R^{i}_{j}))|$$

We know that, 
$\sum_{p=1}^{m}|P(D_{\alg}(t-1, Bl(p)))|=|\alg(t-1)|$
Hence, by Lemma~\ref{size of remainder(1)} and Lemma~\ref{size of remainder(2)}, we know, 

$$\sum_{(i,j)}|P(D_{\alg}(t-1, R^{i}_{j}))| \leq (2z+2)|\alg(t-1)|$$, where the sum runs over all pairs $(i,j)$ with $1\leq i \leq c$ and $1\leq j \leq m_{i^*}$.

Also, 
$$\sum_{(i,j)}|P(D_{\alg}(t-1, P^{i}_{j}))| = c|\alg(t-1)|$$, where the sum runs over all pairs $(i,j)$ with $1\leq i \leq c$ and $1\leq j \leq m_{i^*}$.

Hence, we have,
$$\sum_{(i,j)}|P(D_{\alg}(t-1, Q^{i}_{j}))| \leq (c+2z+2)\alg(t-1) < (c+\frac{c\varepsilon}{4})|\alg(t-1)|$$, where the sum runs over all pairs $(i,j)$ with $1\leq i \leq c$ and $1\leq j \leq m_{i^*}$.


So we have $\sum_{(i,j)}|P^*(\cDoptin(t, P^{i}_{j}))|>\sum_{(i,j)}|P(D_{\alg}(t-1, Q^{i}_{j}))|$, where the sum runs over all pairs $(i,j)$ with $1\leq i \leq c$ and $1\leq j \leq m_{i^*}$. Hence the result follows.



\end{proof}


Now, set $\Snew=\cDoptin(t, P^{i^*}_{j^*})$ and $\Sold=D_{\alg}(t-1, Q^{i^*}_{j^*})$ in algorithm \textsc{SAS-MC}. We have $\cDalg(t)=\cDalg(t-1) \cup \Snew \setminus \Sold$. Now from the definition of $P^*$, we know that any point in $P(\cDalg(t-1)) \setminus P(\Sold)$ is not present in $P^*(\Snew)$. Now by Lemma~\ref{Swapping increase number of point}, we have,  $|P^*(\cDoptin(t, P^{i^*}_{j^*}))|> |P(D_{\alg}(t-1, Q^{i^*}_{j^*}))|$. Hence we have $$|P(\cDalg(t))|\geq |P(\cDalg(t-1))| + |P^*(\Snew)|- |P(\Sold)|>|P(\cDalg(t-1))| \geq |P(\cDalg(t-1))|+1 $$. Also by Lemma~\ref{possiblereplacement}, we have $|\Snew| \leq |\Sold|$. Finally since, $Q^{i^*}_{j^*})$ is a union of (c+z) blocks. So by property 1 of a block we have $$|D_{\alg}(t-1, Q^{i^*}_{j^*})|\leq (c+z)\frac{(c^*+2)}{\varepsilon^2}=O(\frac{1}{\varepsilon^3})$$. Thus the selected $\Snew$ and $\Sold$ are sets of unit disks with "good" property as desired in algorithm \textsc{SAS-MC}. Thus proving the existence of SAS with $f(\varepsilon)=O(\frac{1}{\varepsilon^3})$.


%\begin{lemma} \label{Swapping is stable}
 %  There exists $i,j$ with $1\leq i \leq c$ and $1\leq j\leq m_i$ such that the number of points covered by the unit disks in $\cDoptin(t, P^i_j)$ is strictly greater than the number of points covered by the unit disks in $D_{\alg}(t-1, Q^i_j)$.
%\end{lemma}

%\begin{proof}
 
%\end{proof}
